Plain-Det: A Plain Multi-Dataset Object Detector

Recent advancements in large-scale foundational models have sparked widespread interest in training highly proficient large vision models. A common consensus revolves around the necessity of aggregating extensive, high-quality annotated data. However, given the inherent challenges in annotating dense tasks in computer vision, such as object detection and segmentation, a practical strategy is to combine and leverage all available data for training purposes. In this work, we propose Plain-Det, which offers flexibility to accommodate new datasets, robustness in performance across diverse datasets, training efficiency, and compatibility with various detection architectures. We utilize Def-DETR, with the assistance of Plain-Det, to achieve a mAP of 51.9 on COCO, matching the current state-of-the-art detectors. We conduct extensive experiments on 13 downstream datasets and Plain-Det demonstrates strong generalization capability. Code is release at https://github.com/ChengShiest/Plain-Det

==> sec/3_method_sc.tex <==

\section{Our Method}

\label{sec:method}
\begin{figure*}[ht]
    \centering
\includegraphics[width=0.99\textwidth]{fig/t_framework.png} 
    % \vspace{-6mm}
    \caption{XXXX.}
\label{fig:fig2} 
\end{figure*}

In a nutshell, we propose a general framework and training strategy for multi-dataset detection without restriction to specific detection architectures, which implies that our framework is compatible with various detection families.  
% This implies that our framework is compatible with various detection families, such as RCNN or DETR, as long as they adhere to a query-based approach, with only minor adjustments required for the detectors.
In Sec~\ref{subsec:pre}, we first introduce the preliminaries on object detectors and three primary components of multi-dataset training. In the upcoming sections, we offer an extensive elucidation of each aspect, each addressing a specific question related to multi-dataset training. Section~\ref{subsec:Label} delineates the construction of the label loss. Section~\ref{subsec:Query} expounds on the selection and enhancement of detector models. Lastly, Section~\ref{subsec:uncertainty} delves into the sampling of multi-dataset data.
% \textcolor{blue}{
% In the subsequent sections, we provide a detailed exposition of each, namely Sec~\ref{subsec:uncertainty} on Hardness-Guided Data Sampling, Sec~\ref{subsec:Query} on Class-Aware Query Compositor and Sec~\ref{subsec:Label} on Bias-Aware Label Space Regularization.}

\subsection{Preliminaries}
\label{subsec:pre}
\textbf{Query-based object detector.} Through a set of learnable queries, query-based approaches~\TODO{cite} achieve sparse object output, thus circumventing the need for pre-defined anchor boxes or hand-crafted post-processing procedures. 
Its elegant design, robust performance, and modular architecture have propelled query-based methods to a prominent position in the current landscape of object detection.
Our approach is compatible with all query-based methods. Therefore, we offer a concise and abstract formulation of the workflow of all query-based methods for ease of subsequent comprehension. 
A typical query-based detector consists of three components: a set of learnable queries, an image encoder (e.g. attention mechanism~\TODO{cite} in DETR~\TODO{cite} or CNN~\TODO{cite} in Sparse-RCNN~\TODO{cite}), and a decoder (e.g. cross-attention mechanism~\TODO{cite} in DETR~\TODO{cite} or several dynamic heads~\TODO{cite} in Sparse-RCNN~\TODO{cite}). 
Given an image $I$ and a set of learnable queries $Q$, the image encoder extracts the image features, which are fed to the decoder with the queries. The decoder then employs the image features to refine the query features and regress class $C$ and bounding box $B$ through the refined query features. 

\noindent\textbf{Multi-dataset object detection.} Different from single dataset object detection, multi-dataset training involves the consideration of M datasets, each with its distinct label space. Distinct datasets exhibit varying data distributions, and the presence of domain gaps contributes to differences in their learning complexities. For instance, COCO~\TODO{cite} and LVIS~\TODO{cite} both include approximately 10 million images from the same domain. However, COCO annotates only 80 common objects, whereas LVIS covers 1203 categories. On the other hand, Object365~\TODO{cite} comprises 365 categories, significantly fewer than LVIS, yet it boasts nearly ten times the amount of image data. The natural divergence in training data across different datasets leads us to address three fundamental questions. 
\textcolor{violet}{\ding{182}} How can we ensure consistent training and efficiently leverage the advantages of distinct datasets, considering the combination of numerous datasets and a large number of labels? \textcolor{violet}{\ding{183}} How should we go about selecting and enhancing a detector based on the varying performance of different types of detectors when confronted with large-scale and complex distribution datasets?
\textcolor{violet}{\ding{184}} How should we address the issue of imbalanced dataset sizes, data distribution, and training difficulty between various datasets? 
We will address each of these questions in the upcoming sections. 

\subsection{Construct Label Space and Class Loss}
\label{subsec:Label}
% label 拼接 -》 多头
% text embed 干扰
Next, we consider the methodology for calculating class losses among diverse datasets in a multi-dataset configuration. One possible solution is to directly concatenate the data. Still, as the size of the datasets increases, the total number of classes could become enormous and difficult to optimize (For instance, when we concatenate datasets like COCO, Object365, and LVIS, the number of classes swells to nearly two thousand.). Following UniDet~\TODO{cite}, we adopt a partitioned head as shown in Fig~\TODO{cite}. This implies that during training, the labels from one dataset are invisible to the other dataset. To address this disparity and provide mutual improvement of common classes or knowledge across diverse datasets, we utilize fixed text embeddings from pre-trained VLM~\TODO{cite} as partitioned class heads. The text embedding is generated by:
\begin{equation}
    L_C = \text{Text Enc} (\text{Prompt Enc}(C)),
\end{equation}
where Prompt Enc is to construct text ``$\textit{the photo is}$ [category name]'' based on category name from $C$ and Text Enc is frozen text encoder from VLM. As shown in Fig~\TODO{cite}, during testing, we find that The coupling relationships between the vast majority of text embeddings adhere to visual or semantic associations. However, there are instances where the similarity between certain categories and their coupling to all other categories is exceptionally high, such as ``person.'' Our analysis suggests that this might be due to data distribution reasons during VLM pre-training, where some nouns might not have learned a strong visual association. For instance, the concept of a person might be overly prevalent in the pre-training data, leading to a network structure with inherent biases. We regularize the text embedding by splitting the model basis as follows:
\begin{equation}
    L =\text{Norm}(L_C - L_{\textit{``''}}),
\end{equation}
where $L_{\textit{``''}}$ is just the query feature generated by an empty string, and the norm is l2 norm. As shown in Fig~\TODO{cite}, after regularization, we position our label space within a more suitable range.
\subsection{Class-Aware Query Compositor}
\label{subsec:Query}
% How to choose a detector? How do you think you could improve your detector?
% 发现 init query 和 类别相关


As shown in Anchor-Detr~\TODO{cite} and Conditional-Detr~\TODO{cite}, a context query often contains the prior knowledge regarding the location of objects. Based on \TODO{Fig}, we propose that in multi-dataset training, queries play an additional role in balancing the distribution disparities among datasets. Based on this observation, we introduce a novel query initialization method. Given an image $I$ and the corresponding dataset label embedding $L$ $\in$ $\mathbb{R}^{m \times d}$, where $m$ is the number of class and $d$ is the dimension, we first construct a basis query embedding $\mathcal{Q}^b$ based on the label embedding as follows:
\begin{equation}
    \mathcal{Q}^b = \text{MLP} (\text{Norm}(L)),
\end{equation}
where Norm is l2 norm. Subsequently, extract the image features through an image encoder, followed by a max-pooling operation over all patches. Afterward, directly regress the weights as follows:
\begin{equation}
    \mathcal{W} = \text{MLP} (\text{Max-Pool}(\text{Image Enc}(I))),
\end{equation}
where $ \mathcal{W}$ $\in$ $\mathbb{R}^{k \times m}$ and $k$ is the number of final query fed into decoder. Following this, composite the class-aware query by:
\begin{equation}
    \mathcal{Q}^c = \mathcal{W} \mathcal{Q}^b,
\end{equation}
As shown above, our modifications are solely related to query initialization. Therefore, all query-based methods can be updated to class-aware using this approach.


\subsection{Hardness-Guided Data Sampling}
\label{subsec:uncertainty}
Initially, we focus on a single dataset, aiming to minimize box $B$ and label $C$ losses on image $I$ by
% $$
% \min _{f} \mathbb{E}_{(I, B, C) \sim D}[\ell(f(I), B, C)],
% $$

\begin{equation}
\underset{f}{\operatorname{argmin}}
\quad
 \mathbb{E}_{(I, B, C) \sim D}[\ell(f(I), B, C)],
\end{equation}
where singular dataset's $I$, $B$, and $C$ adhere to an identical distribution, denoted as $D$. The loss function $\ell$ is typically the cross-entropy loss for the label and the generalized intersection over union (GIOU) loss for the box. 
Let's consider the multi-dataset training, as we show in Figure~\TODO{fig}, and it is noteworthy that distinct datasets exhibit entirely disparate \textcolor{red}{convergence curves}. Moreover, there is a significant difference in the distribution of data, denoted as $D$, which includes variances in the amount of data, the level of granularity in annotations, and the domain of the images. The optimization for multi-dataset can be viewed as follows:
\begin{equation}
\underset{f}{\operatorname{argmin}}
\quad
 \mathbb{E}_{(I, B, C) \sim D_1 \cup D_2 \cup ... \cup D_M}[\ell(f(I), B, C)],
\end{equation}
where different datasets adhere to different distributions. When there is a large difference across datasets, the optimization process for training with many datasets might easily degenerate by focusing solely on optimizing one dataset. This might happen because one dataset is very complex or has a lot of data. To avoid the degeneration issue, we propose to resample the data distribution $D$ to rebalance the expected loss $\mathbb{E}_{(I, B, C) \sim D}$. 
\textcolor{red}{We first compute the mean of bbox loss $L_1$ $L_2$...$L_n$  before a new epoch for every dataset.
Then we calculate the online sampling weight $w_1$ $w_2$ ...$w_n$ by}
\begin{equation}
    {\{w_{1...n}\}}=1+[
        \frac{\max\{S_{1...n}\}}{\{S_{1..n}\}}
        (\frac{\{L_{1...n}\}}{\min\{L_{1..n}\}}-1)
    ]^\alpha
\end{equation}
Where $S_i$ means the number of images in the \textit{ith} dataset.

==> tables/rn50_coco.tex <==
\begin{tabular}{lccc}\toprule
        Method  & \makecell{multi\\datasets} & \makecell{\textcolor{gray}{COCO train}\\ epoch} & \makecell{\textcolor{gray}{COCO val}\\ AP$^{\text{box}}$} \\\midrule
        Mask RCNN~\cite{he2017mask} & \xmark & 36 &39.8 \\ 
        RegionCLIP~\cite{zhong2021regionclip}  & \cmark & - &42.7 \\ \hline
        CenterNet2~\cite{zhou2021probabilistic}  & \xmark & 12  &42.9\\ 
        Detic\cite{zhou2022detecting}  & \cmark & - & 42.4 \\ 
        ScaleDet~\cite{scaledet} & \cmark & - & 47.1 \\ \hline
        Sparse RCNN\cite{sparsercnn}   & \xmark & 12/36 & 43.0/45.0 \\ 
         + Det-Hub~\cite{detectionhub} & \cmark & 12 & 45.3 \\ 
        \rowcolor[HTML]{efefef} + Ours & \cmark & 12 & 45.1 \\ \hline
        Def-DETR\cite{zhu2020deformable}   & \xmark & 300 & 45.5 \\ 
        \rowcolor[HTML]{efefef} + Ours & \cmark & 12 & 51.9 \\ 
        \bottomrule
        \end{tabular}

==> tables/s_abla.tex <==
\begin{tabular}{lc|ccc|c}
\toprule
 & \texttt{Sampler}  & C\cite{coco}&  L\cite{gupta2019lvis}  & O365~\cite{shao2019objects365}& mAP \\  
\hline 4  & \xmark &43.5  &26.8  &25.5  &31.9 \\
\rowcolor[HTML]{efefef}5 & \cmark & \textbf{47.1} &\textbf{32.4}  &\textbf{25.6}  &\textbf{35.0} \\
\hline
\end{tabular}

==> tables/table1.tex <==
\begin{table}[ht]
    \centering
    \caption{Toy Experiment}
    \setlength{\tabcolsep}{0.75mm}{
    \begin{tabular}{l|c|cccc}
  \toprule
Method& Query & C&L& C* & L*\\ \hline
Def-DETR-two &$\times$& 42.8& 27.2& 38.6{\color{ForestGreen}{ 4.2$\downarrow$}}& 24.5{\color{ForestGreen}{ 2.7$\downarrow$}}\\
Def-DETR &$\checkmark$& 45.5& 28.2& 41.6{\color{ForestGreen}{ 3.9$\downarrow$}}& 27.0{\color{ForestGreen}{ 1.2$\downarrow$}}\\
Fast-RCNN &$\times$&34.9& 19.8&33.3{\color{ForestGreen}{ 1.6$\downarrow$}}& 15.1{\color{ForestGreen}{ 4.7$\downarrow$}} \\
Sparse-RCNN &$\checkmark$&38.3&20.9&37.5{\color{ForestGreen}{ 0.8$\downarrow$}}&19.1{\color{ForestGreen}{ 1.8$\downarrow$}}\\
\bottomrule
\end{tabular}}
    \label{tab:my_label}
\end{table}


==> tables/table6_13_.tex <==
\begin{table*}[h]
  \centering
  \caption{{\bf Results of fine-tuning transfer on 13 individual datasets on ODinW.} 
  R denotes ResNet50 backbone and T denotes Swin-Tiny.
  }
  \resizebox{0.95\linewidth}{!}{%
  \begin{tabular}{l | c | ccccccccccccc c}
    \toprule
    % Model & Model Type & \#Data & AerialDrone & Aquarium & Rabbits & EgoHands & Mushrooms & Packages & PascalVOC & pistols & pothole & Raccoon & Shellfish & Thermal & Vehicles & \cellcolor[HTML]{efefef} mAP \\
    Model  & \#Data & \#1 & \#2 & \#3 & \#4 & \#5 & \#6 & \#7 & \#8 & \#9 & \#10 & \#11 & \#12 & \#13 & \cellcolor[HTML]{efefef} mAP \\
    \midrule
    GLIP-T\cite{Li_2022_CVPR} & 5.5M & 31.2 & 52.5 & 70.8 & 78.7 & 88.1 & 75.6 & 62.3 &\textcolor{gray}{71.2} & 58.7 & 61.4 & 51.4 & 76.7 & 65.3 & \cellcolor[HTML]{efefef}64.4 \\
    GLIPv2-T\cite{zhang2022glipv2}  & 5.5M & 30.2 & 52.5 & 74.8 & 80.0 & 88.1 & 74.3 & 66.4 & \textcolor{gray}{73.0} & 60.1 & 63.7 & 54.4 & 63.0 & 83.5 & \cellcolor[HTML]{efefef}65.9 \\ 
    \midrule
    Detic-R\cite{zhou2022detecting}  & 12.6M & 43.1 & 49.5 & 72.2 & 78.0 & 91.0 & 70.0 & 49.1 & \textcolor{gray}{99.9} & 45.8 & 66.2 & 38.0 & 82.3 & 52.4 & \cellcolor[HTML]{efefef}58.1 \\
    % Detic-B\cite{zhou2022detecting}  & 12.6M & 44.3 & 51.9 & 76.2 & 78.2 & 89.8 & 75.1 & 96.4 & 99.9 & 50.7 & 64.3 & 47.6 & 82.4 & 54.4 & \cellcolor[HTML]{efefef}67.6 \\
    % \midrule
    ScaleDet-R~\cite{scaledet}  & 3.6M & 42.6 & 49.2 & 72.3 & 78.1 & 89.8 & 75.7 & 91.8 & \textcolor{gray}{99.9} & 47.4 & 67.5 & 40.0 & 82.1 & 54.5 & \cellcolor[HTML]{efefef}65.9 \\
    % ScaleDet-T  & 3.6M & 46.0 & 52.1 & 73.1 & 79.2 & 91.6 & 76.5 & 95.1 & 99.9 & 50.1 & 65.6 & 47.8 & 83.1 & 54.7 & \cellcolor[HTML]{efefef}67.9 \\ 
    \midrule
    \rowcolor[HTML]{efefef} Ours-R  & 3.6M & 36.6 & 49.7 & 77.2 & 75.7 & 92.8 &76.2 & 67.1 & \textcolor{gray}{75.7} & 53.5 &69.6 & 58.7 &83.6 & 61.7 & \bf 66.9 \\
    \bottomrule
  \end{tabular}
  }  
  \label{tab:odinw13}

\end{table*}


% \begin{table*}[t]
%   \centering
%   \caption{{\bf Results of fine-tune transfer on other 8 individual datasets on ODinW.} 
%   R, T, B: ResNet50, Swin-Tiny, Swin-Base Transformer as backbone. 
%   Metric: mAP over 8 datasets.
%   }
%   \resizebox{0.7\linewidth}{!}{%
%   \begin{tabular}{l | c | cccccccc c}
%     \toprule
%     % Model & Model Type & \#Data & AerialDrone & Aquarium & Rabbits & EgoHands & Mushrooms & Packages & PascalVOC & pistols & pothole & Raccoon & Shellfish & Thermal & Vehicles & \cellcolor[HTML]{efefef} mAP \\
%     Model  & \#Data & \#1 & \#2  & \#3 & \#4 & \#5  & \#6 &\#7& \#8 & \cellcolor[HTML]{efefef} mAP \\
%     \midrule
%     GLIP-T\cite{Li_2022_CVPR} & 5.5M & 31.2 &70.8 &  88.1 & 75.6 & 62.3 &58.7 & 51.4 &65.3 & \cellcolor[HTML]{efefef}62.9 \\
%     % GLIPv2-T\cite{zhang2022glipv2}  & 5.5M & 30.2 &74.8 &  88.1 & 74.3 & 66.4& 60.1 &54.4 & 83.5 & \cellcolor[HTML]{efefef}66.5 \\ 
%     % \midrule
%     Detic-R\cite{zhou2022detecting}  & 12.6M & 43.1 &72.2 &91.0 & 70.0 & 49.1 & 45.8 &38.0 &52.4 & \cellcolor[HTML]{efefef}57.7 \\
%     % Detic-B\cite{zhou2022detecting}  & 12.6M & 44.3 &76.2 &89.8 & 75.1 & 96.4 & 50.7 &47.6 &54.4 & \cellcolor[HTML]{efefef}66.8 \\
%     % \midrule
%     ScaleDet-R  & 3.6M & 42.6& 72.3  & 89.8 & 75.7 & 91.8& 47.4 & 40.0 & 54.5 & \cellcolor[HTML]{efefef}64.3 \\
%     % ScaleDet-T  & 3.6M & 46.0& 73.1& 91.6 & 76.5 & 95.1& 50.1& 47.8 &54.7 & \cellcolor[HTML]{efefef}66.9 \\ 
%     \midrule
%     \rowcolor[HTML]{efefef} Ours-R  & 3.6M & 36.6& 77.2& 92.8 &76.2 & 67.1& 53.5 & 58.7& 61.7 & \bf 65.5 \\
%     \bottomrule
%   \end{tabular}
%   }  
%   \label{tab:odinw12}

% \end{table*}

==> tables/vit_coco.tex <==
\begin{tabular}{lccc}\toprule
        Method  & \makecell{BackBone} & \makecell{enc.\\hparams}  & \makecell{\textcolor{gray}{COCO val}\\ AP$^{\text{box}}$} \\\midrule
        ScaleDet\cite{scaledet} & Swin-B & 88M & 58.8  \\
        GLIP-L & Swin-L & 284M & 60.8 \\
        CO-DETR\cite{detr} & Swin-L & 284M & 64.1 \\
        DINO\cite{dino} & Swin-L & 218M & 63.1  \\
        \rowcolor[HTML]{efefef} Ours & Swin-L & 218M  & - \\
        \bottomrule
        \end{tabular}
